Realization of Causal Representation Learning to Adjust Confounding Bias in Latent Space

Causal DAGs(Directed Acyclic Graphs) are usually considered in a 2D plane. Edges indicate causal effects' directions and imply their corresponding time-passings. Due to the natural restriction of statistical models, effect estimation is usually approximated by averaging the individuals' correlations, i.e., observational changes over a specific time. However, in the context of Machine Learning on large-scale questions with complex DAGs, such slight biases can snowball to distort global models - More importantly, it has practically impeded the development of AI, for instance, the weak generalizability of causal models. In this paper, we redefine causal DAG as \emph{do-DAG}, in which variables' values are no longer time-stamp-dependent, and timelines can be seen as axes. By geometric explanation of multi-dimensional do-DAG, we identify the \emph{Causal Representation Bias} and its necessary factors, differentiated from common confounding biases. Accordingly, a DL(Deep Learning)-based framework will be proposed as the general solution, along with a realization method and experiments to verify its feasibility.

==> acmart.tex <==

IEEEabrv.bib
V1.12 (2007/01/11)
Copyright (c) 2002-2007 by Michael Shell
See: http://www.michaelshell.org/
for current contact information.

BibTeX bibliography string definitions of the ABBREVIATED titles of
IEEE journals and magazines and online publications.

This file is designed for bibliography styles that require 
abbreviated titles and is not for use in bibliographies that
require full-length titles.

Support sites:
http://www.michaelshell.org/tex/ieeetran/
http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
and/or
http://www.ieee.org/

Special thanks to Laura Hyslop and ken Rawson of IEEE for their help
in obtaining the information needed to compile this file. Also,
Volker Kuhlmann and Moritz Borgmann kindly provided some corrections
and additions.

*************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEabrv.bib, IEEEfull.bib, IEEEexample.bib,
                   IEEEtran.bst, IEEEtranS.bst, IEEEtranSA.bst,
                   IEEEtranN.bst, IEEEtranSN.bst, IEEEtran_bst_HOWTO.pdf
*************************************************************************


USAGE:

\bibliographystyle{mybstfile}
\bibliography{IEEEabrv,mybibfile}

where the IEEE titles in the .bib database entries use the strings
defined here. e.g.,


   journal = IEEE_J_AC,


to yield "{IEEE} Trans. Automat. Contr."


IEEE uses abbreviated journal titles in their bibliographies -
this file is suitable for work that is to be submitted to the IEEE.


For work that requires full-length titles, you should use the full
titles provided in the companion file, IEEEfull.bib.


** NOTES **

 1. Journals have been grouped according to subject in order to make it
    easier to locate and extract the definitions for related journals - 
    as most works use references that are confined to a single topic.
    Magazines are listed in straight alphabetical order.

 2. String names are closely based on IEEE's own internal acronyms.
 
 3. Abbreviations follow IEEE's style.

 4. Older, out-of-print IEEE titles are included (but not including titles
    dating prior to IEEE's formation from the IRE and AIEE in 1963).

 5. The following NEW/current journal definitions have been disabled because
    their abbreviations have not yet been verified:
    
    STRING{IEEE_J_CBB        = "{IEEE/ACM} Trans. Comput. Biology Bioinformatics"}
    STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
    STRING{IEEE_J_DSC        = "{IEEE} Trans. Dependable Secure Comput."}
    STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
    
 6. The following OLD journal definitions have been disabled because
    their abbreviations have not yet been found/verified:

    STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
    STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}

If you know what the proper abbreviation is for a string in #5 or #6 above,
email me and I will correct them in the next release.





IEEE Journals 



aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}



circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
in 2004 CASI and CASII renamed part title to CASI_RP and CASII_EB, respectively.
@STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}



components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}



coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
disabled till definition is verified
STRING{IEEE_J_DSC         = "{IEEE} Trans. Dependable Secure Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



computer graphics, imaging, and multimedia
@STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
in 1989 JRA became RA
in August 2004, RA split into ASE and RO
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_GRSL       = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}



education, engineering, history, IEEE, professional
disabled till definition is verified
STRING{IEEE_J_CJECE       = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
disabled till definition is verified
STRING{IEEE_J_EWS         = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
IEEE seems to want "Compon." here, not "Comp."
@STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Tech."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



energy and power
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PEL        = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}



industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
disabled till definition is verified
STRING{IEEE_J_BCTV        = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}



instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



insulation and materials
@STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Electr. Insul."}



mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}



medical and biological
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
disabled till definition is verified
STRING{IEEE_J_CBB         = "{IEEE/ACM} Trans. Comput. Biology Bioinformatics"}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehabil. Eng."}



 optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_JLT        = "J. Lightw. Technol."}



physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



reliability
IEEE seems to want "Mat." here, not "Mater."
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond. Manuf."}



sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}






IEEE Magazines 



@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NET        = "{IEEE} Netw."}
IEEE's editorial manual lists "Pers. Commun.", 
but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun. Mag."}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}






IEEE Online Publications 



@STRING{IEEE_O_CSTO        = "{IEEE} Commun. Surveys Tuts."}
disabled till definition is verified
STRING{IEEE_O_DSO          = "{IEEE} Distrib. Syst. Online"}


@article{wood2015lesson,
  title={The lesson of causal discovery algorithms for quantum correlations: Causal explanations of Bell-inequality violations require fine-tuning},
  author={Wood, Christopher J and Spekkens, Robert W},
  journal={New Journal of Physics},
  volume={17},
  number={3},
  pages={033002},
  year={2015},
  publisher={IOP Publishing}
}

@article{vukovic2022causal,
  title={Causal Discovery in Manufacturing: A Structured Literature Review},
  author={Vukovi{\'c}, Matej and Thalmann, Stefan},
  journal={Journal of Manufacturing and Materials Processing},
  volume={6},
  number={1},
  pages={10},
  year={2022},
  publisher={MDPI}
}

@article{ombadi2020evaluation,
  title={Evaluation of methods for causal discovery in hydrometeorological systems},
  author={Ombadi, Mohammed and Nguyen, Phu and Sorooshian, Soroosh and Hsu, Kuo-lin},
  journal={Water Resources Research},
  volume={56},
  number={7},
  pages={e2020WR027251},
  year={2020},
  publisher={Wiley Online Library}
}


@inproceedings{zheng2020causal,
  title={Learning sparse nonparametric dags},
  author={Zheng, Xun and Dan, Chen and Aragam, Bryon and Ravikumar, Pradeep and Xing, Eric},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3414--3425},
  year={2020},
  organization={PMLR}
}

@article{lachapelle2019gradient,
  title={Gradient-based neural dag learning},
  author={Lachapelle, S{\'e}bastien and Brouillard, Philippe and Deleu, Tristan and Lacoste-Julien, Simon},
  journal={arXiv:1906.02226},
  year={2019}
}

@article{luo2020causal,
  title={When causal inference meets deep learning},
  author={Luo, Yunan and Peng, Jian and Ma, Jianzhu},
  journal={Nature Machine Intelligence},
  volume={2},
  number={8},
  pages={426--427},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{scheines1997introduction,
  title={An introduction to causal inference},
  author={Scheines, Richard},
  year={1997},
  publisher={Carnegie Mellon University}
}

@article{glymour2019review,
  title={Review of causal discovery methods based on graphical models},
  author={Glymour, Clark and Zhang, Kun and Spirtes, Peter},
  journal={Frontiers in genetics},
  volume={10},
  pages={524},
  year={2019},
  publisher={Frontiers Media SA}
}

@article{ma2018using,
  title={Using deep learning to model the hierarchical structure and function of a cell},
  author={Ma, Jianzhu and Yu, Michael Ku and Fong, Samson and Ono, Keiichiro and Sage, Eric and Demchak, Barry and Sharan, Roded and Ideker, Trey},
  journal={Nature methods},
  volume={15},
  number={4},
  pages={290--298},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{lin2017using,
  title={Using neural networks for reducing the dimensions of single-cell RNA-Seq data},
  author={Lin, Chieh and Jain, Siddhartha and Kim, Hannah and Bar-Joseph, Ziv},
  journal={Nucleic acids research},
  volume={45},
  number={17},
  pages={e156--e156},
  year={2017},
  publisher={Oxford University Press}
}

@article{li2020teaching,
  title={Teaching deep learning causal effects improves predictive performance},
  author={Li, Jia and Jia, Xiaowei and Yang, Haoyu and Kumar, Vipin and Steinbach, Michael and Simon, Gyorgy},
  journal={arXiv preprint arXiv:2011.05466},
  year={2020}
}


@article{scholkopf2021toward,
  title={Toward causal representation learning},
  author={Sch{\"o}lkopf, Bernhard and Locatello, Francesco and Bauer, Stefan and Ke, Nan Rosemary and Kalchbrenner, Nal and Goyal, Anirudh and Bengio, Yoshua},
  journal={Proceedings of the IEEE},
  volume={109},
  number={5},
  pages={612--634},
  year={2021},
  publisher={IEEE}
}

@article{li2020causal,
  title={Causal discovery in physical systems from videos},
  author={Li, Yunzhu and Torralba, Antonio and Anandkumar, Anima and Fox, Dieter and Garg, Animesh},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={9180--9192},
  year={2020}
}

@article{zhong2016overview,
  title={An overview on data representation learning: From traditional feature learning to recent deep learning},
  author={Zhong, Guoqiang and Wang, Li-Na and Ling, Xiao and Dong, Junyu},
  journal={The Journal of Finance and Data Science},
  volume={2},
  number={4},
  pages={265--278},
  year={2016},
  publisher={Elsevier}
}

@article{bengio2012unsupervised,
  title={Unsupervised feature learning and deep learning: A review and new perspectives},
  author={Bengio, Yoshua and Courville, Aaron C and Vincent, Pascal},
  journal={CoRR, abs/1206.5538},
  volume={1},
  number={2665},
  pages={2012},
  year={2012}
}

@article{Nearing2021,
  title={What role does hydrological science play in the age of machine learning?},
  author={Nearing, Grey S and Kratzert, Frederik and Sampson, Alden Keefe and Pelissier, Craig S and Klotz, Daniel and Frame, Jonathan M and Prieto, Cristina and Gupta, Hoshin V},
  journal={Water Resources Research},
  volume={57},
  number={3},
  pages={e2020WR028091},
  year={2021},
  publisher={Wiley Online Library}
}

@article{Shen2018,
  title={A transdisciplinary review of deep learning research and its relevance for water resources scientists},
  author={Shen, Chaopeng},
  journal={Water Resources Research},
  volume={54},
  number={11},
  pages={8558--8593},
  year={2018},
  publisher={Wiley Online Library}
}

@article{debate_Goodwill2020,
  title={Debates—Does information theory provide a new paradigm for Earth science? Causality, interaction, and feedback},
  author={Goodwell, Allison E and Jiang, Peishi and Ruddell, Benjamin L and Kumar, Praveen},
  journal={Water Resources Research},
  volume={56},
  number={2},
  pages={e2019WR024940},
  year={2020},
  publisher={Wiley Online Library}
}

@article{Singh2019,
  title={A Granger causality analysis of groundwater patterns over a half-century},
  author={Singh, Nitin K and Borrok, David M},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--8},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{hess-18-Kratzert,
  title={Rainfall--runoff modelling using long short-term memory (LSTM) networks},
  author={Kratzert, Frederik and Klotz, Daniel and Brenner, Claire and Schulz, Karsten and Herrnegger, Mathew},
  journal={Hydrology and Earth System Sciences},
  volume={22},
  number={11},
  pages={6005--6022},
  year={2018},
  publisher={Copernicus GmbH}
}

@article{Kratzert2019,
  title={Towards learning universal, regional, and local hydrological behaviors via machine learning applied to large-sample datasets},
  author={Kratzert, Frederik and Klotz, Daniel and Shalev, Guy and Klambauer, G{\"u}nter and Hochreiter, Sepp and Nearing, Grey},
  journal={Hydrology and Earth System Sciences},
  volume={23},
  number={12},
  pages={5089--5110},
  year={2019},
  publisher={Copernicus GmbH}
}

@article{2022Li_Soil,
  title={Sequence-to-Sequence Learning for Prediction of Soil Temperature and Moisture},
  author={Li, Xiaojie and Tang, Jian and Yin, Chengxiang},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={19},
  pages={1--5},
  year={2022},
  publisher={IEEE}
}

@article{caliendo2008some,
  title={Some practical guidance for the implementation of propensity score matching},
  author={Caliendo, Marco and Kopeinig, Sabine},
  journal={Journal of economic surveys},
  volume={22},
  number={1},
  pages={31--72},
  year={2008},
  publisher={Wiley Online Library}
}


@article{goudet2017causal,
  title={Causal generative neural networks},
  author={Goudet, Olivier and Kalainathan, Diviyan and Caillou, Philippe and Guyon, Isabelle and Lopez-Paz, David and Sebag, Mich{\`e}le},
  journal={arXiv preprint arXiv:1711.08936},
  year={2017}
}

@article{reisach2021beware,
  title={Beware of the simulated dag! varsortability in additive noise models},
  author={Reisach, Alexander G and Seiler, Christof and Weichwald, Sebastian},
  journal={arXiv preprint arXiv:2102.13647},
  year={2021}
}

@article{kaiser2021unsuitability,
  title={Unsuitability of NOTEARS for causal graph discovery},
  author={Kaiser, Marcus and Sipos, Maksim},
  journal={arXiv preprint arXiv:2104.05441},
  year={2021}
}

@article{zheng2018dags,
  title={Dags with no tears: Continuous optimization for structure learning},
  author={Zheng, Xun and Aragam, Bryon and Ravikumar, Pradeep K and Xing, Eric P},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}

@inproceedings{germain2015made,
  title={Made: Masked autoencoder for distribution estimation},
  author={Germain, Mathieu and Gregor, Karol and Murray, Iain and Larochelle, Hugo},
  booktitle={International conference on machine learning},
  pages={881--889},
  year={2015},
  organization={PMLR}
}

@inproceedings{larochelle2011neural,
  title={The neural autoregressive distribution estimator},
  author={Larochelle, Hugo and Murray, Iain},
  booktitle={Proceedings of the fourteenth international conference on artificial intelligence and statistics},
  pages={29--37},
  year={2011},
  organization={JMLR Workshop and Conference Proceedings}
}

@article{dinh2016density,
  title={Density estimation using real nvp},
  author={Dinh, Laurent and Sohl-Dickstein, Jascha and Bengio, Samy},
  journal={arXiv preprint arXiv:1605.08803},
  year={2016}
}


@article{ke2019learning,
  title={Learning neural causal models from unknown interventions},
  author={Ke, Nan Rosemary and Bilaniuk, Olexa and Goyal, Anirudh and Bauer, Stefan and Larochelle, Hugo and Sch{\"o}lkopf, Bernhard and Mozer, Michael C and Pal, Chris and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1910.01075},
  year={2019}
}

@inproceedings{young2020learning,
  title={Learning Latent Causal Structures with a Redundant Input Neural Network},
  author={Young, Jonathan D and Andrews, Bryan and Cooper, Gregory F and Lu, Xinghua},
  booktitle={Proceedings of the 2020 KDD Workshop on Causal Discovery},
  pages={62--91},
  year={2020},
  organization={PMLR}
}

@incollection{goudet2018learning,
  title={Learning functional causal models with generative neural networks},
  author={Goudet, Olivier and Kalainathan, Diviyan and Caillou, Philippe and Guyon, Isabelle and Lopez-Paz, David and Sebag, Michele},
  booktitle={Explainable and interpretable models in computer vision and machine learning},
  pages={39--80},
  year={2018},
  publisher={Springer}
}.

@article{lawrence2021data,
  title={Data generating process to evaluate causal discovery techniques for time series data},
  author={Lawrence, Andrew R and Kaiser, Marcus and Sampaio, Rui and Sipos, Maksim},
  journal={arXiv preprint arXiv:2104.08043},
  year={2021}
}

@inproceedings{chattopadhyay2019neural,
  title={Neural network attributions: A causal perspective},
  author={Chattopadhyay, Aditya and Manupriya, Piyushi and Sarkar, Anirban and Balasubramanian, Vineeth N},
  booktitle={International Conference on Machine Learning},
  pages={981--990},
  year={2019},
  organization={PMLR}
}

@article{bica2020estimating,
  title={Estimating the effects of continuous-valued interventions using generative adversarial networks},
  author={Bica, Ioana and Jordon, James and van der Schaar, Mihaela},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={16434--16445},
  year={2020}
}

@article{louizos2017causal,
  title={Causal effect inference with deep latent-variable models},
  author={Louizos, Christos and Shalit, Uri and Mooij, Joris M and Sontag, David and Zemel, Richard and Welling, Max},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{judea2010introduction,
  title={An introduction to causal inference},
  author={Judea, Pearl},
  journal={The International Journal of Biostatistics},
  volume={6},
  number={2},
  pages={1--62},
  year={2010},
  publisher={De Gruyter}
}

@article{miettinen1974confounding,
  title={Confounding and effect-modification},
  author={Miettinen, Olli},
  journal={American Journal of Epidemiology},
  volume={100},
  number={5},
  pages={350--353},
  year={1974},
  publisher={Oxford University Press}
}

@phdthesis{greve2021modeling,
  title={Modeling Flow and Nitrate Losses for Small Watersheds in Southeastern Minnesota},
  author={Greve, Mark},
  year={2021},
  school={University of Minnesota}
}

--
EOF

